Contrastive State Augmentations for Reinforcement Learning-Based Recommender Systems

Learning reinforcement learning (RL)-based recommenders from historical user-item interaction sequences is vital to generate high-reward recommendations and improve long-term cumulative benefits. However, existing RL recommendation methods encounter difficulties (i) to estimate the value functions for states which are not contained in the offline training data, and (ii) to learn effective state representations from user implicit feedback due to the lack of contrastive signals. In this work, we propose contrastive state augmentations (CSA) for the training of RL-based recommender systems. To tackle the first issue, we propose four state augmentation strategies to enlarge the state space of the offline data. The proposed method improves the generalization capability of the recommender by making the RL agent visit the local state regions and ensuring the learned value functions are similar between the original and augmented states. For the second issue, we propose introducing contrastive signals between augmented states and the state randomly sampled from other sessions to improve the state representation learning further. To verify the effectiveness of the proposed CSA, we conduct extensive experiments on two publicly accessible datasets and one dataset collected from a real-life e-commerce platform. We also conduct experiments on a simulated environment as the online evaluation setting. Experimental results demonstrate that CSA can effectively improve recommendation performance.

==> preliminaries.tex <==
% !TEX root = ../main.tex

\section{Preliminaries}
\label{sec:preliminaries}
In this section, we first formulate the basic problem of generating next item recommendations from user sequence. (Sec.~\ref{subsec:Problem formulation}).
Then we introduce the primary settings of RL-based recommendation and the concept of offline RL. (Sec.~\ref{subsec:Reinforcement learning}).

\subsection{Problem formulation}
\label{subsec:Problem formulation}
Assume that we have a set of users and items, denoted by \mathcal{U} and \mathcal{I}, respectively, where $\mathbf{u} \in \mathcal{U}$ denotes a user and $\mathbf{i} \in \mathcal{I}$ denotes an item. Then a user-item interaction sequence can be represented as $\mathit{x}_{\mathit{1:t}}=\{\mathit{x}_{\mathit{1}}, \mathit{x}_{\mathit{2}},...,\mathit{x}_{\mathit{t-1}},\mathit{x}_{\mathit{t}}\}$, where \mathit{t} is the number of interactions and $\mathit{x}_{\mathit{i}}$ is the \mathit{i}-th item that user has interacted with. The goal of sequential recommendation is to predict the next item that the user is likely to interact with given the sequence of previous interactions $\mathit{x}_{\mathit{1:t}}$.
Like~\citep{xin2020self}, we cast this task as a (self-supervised) multi-class classification problem and build a sequential model that generates the classification logits $\mathit{y}_{\mathit{t+1}}=\left[\mathit{y}_{\mathit{1}}, \mathit{y}_{\mathit{2}},...,\mathit{y}_{\mathit{n}}\right] \in \mathbb{R}^\mathit{n}$, where \mathit{n} is the number of candidate items. Typically one can use a generative model \mathit{G} to map the input sequence into a hidden state $\mathbf{s}_{\mathit{t}} = \mathit{G}\left(\mathbf{x}_{\mathit{1:t}}\right)$. This serves as a general encoder function. Based on the obtained hidden state, one can utilize a decoder to map the hidden state to the classification logits as $\mathbf{y}_{\mathit{t+1}} = \mathit{f}\left(\mathbf{s}_{\mathit{t}}\right)$. $\mathit{f}$ is usually defined as a simple fully connected layer or the inner product with candidate item embeddings. \textcolor{blue}{f? is usually defined as a simple fully connected layer or the inner product with candidate item embeddings.} Finally, we can train our recommendation model(agents) by optimizing a loss function based on the logits $\mathbf{y}_{\mathit{t+1}}$, such as cross-entropy loss of the pair-wise ranking loss.

\subsection{Reinforcement Learning}
\label{subsec:Reinforcement learning}
From the perspective of reinforcement learning, next item recommendation is typically framed as a Markov Decision Process (MDP), in which the recommendation agent interacts with the environments (users) by sequentially recommending items to maximize the long-term cumulative rewards. The MDP can be represented by a tuple of the form $\left(\mathcal{S}, \mathcal{A},\rho,\mathit{r}, \gamma,\rho_{\mathit{0}},\right)$, where $\mathcal{S}$ is the state space of the environment. It is modelled by the user's historical interactions with the items. Specifically, the state of the user can be encoded in hidden state by the sequential model \mathcal{G}: $\mathit{s}_{\mathit{t}}=\mathit{G}\left(\mathit{x}_{\mathit{1:t}}\right) \in \mathcal{S}$. $\mathcal{A}$ is the action space. At each timestamp \mathit{t}, the agent selects item $\mathit{i}_{\mathit{t}}$ from candidate item pool and recommends to environment (user). In offline data, we get action at timestamp \mathit{t} from the user-item interaction (i.e. $\mathit{a}_{\mathit{t}}=\mathit{x}_{\mathit{t+1}} \in \mathcal{A}$). $\rho\left(\mathit{s}_{\mathit{t+1}}|\mathit{s}_{\mathit{t}},\mathit{a}_{\mathit{t}}\right)$ is the transition function given the current state and action pair.
$\mathit{r}\left(\mathit{s}_{\mathit{t}}\right)$ is the reward model given the state.
$\gamma$ is the discount factor where $\gamma \in [0, 1]$.
$\rho_{\mathit{0}}$ is the initial state distribution of the MDP. 
A policy $\pi_{\theta}\left(a|s\right)$ which translates the user state $\mathit{s} \in \mathcal{S}$ into a distribution over actions $\mathit{a} \in \mathcal{A}$ is trained to maximize the expected cumulative discount reward in the MDP:
\begin{equation}
    \mathop\mathit{max}_{\substack{\pi_{\theta}}} \mathop\mathbb{E}_{\tau\sim\pi_{\theta}}\left[\mathcal{R}\left(\tau\right)\right], where  \mathcal{R}\left(\tau\right)=\sum_{t=0}^{|\tau|} \gamma^{\mathit{t}} \mathit{r}\left(\mathit{s}_{\mathit{t}}, \mathit{a}_{\mathit{t}} \right)
\end{equation}

As one of the most successful solutions to find the optimal parameters of policy $\pi_{\theta}$, Policy-gradient based approaches (e.g.,REINFORCE~\citep{zhao2018recommendations}) aim at directly learning the mapping function. The gradient of expected accumulated reward with respect to $\theta$ is:
\begin{equation}
    \Delta_{\theta}\mathbb{E}_{\tau\sim\pi_{\theta}}\left[\mathcal{R}\left(\tau\right)\right]=
     \mathbb{E}_{\tau\sim\pi_{\theta}}\left[\mathcal{R}\left(\tau\right)\Delta_{\theta}\log\pi_{\theta}\left(\tau\right)\right]
\end{equation}
Under the recommendation settings, we cannot let a policy interact with users from the beginning to acquire $\tau \sim \pi_{\theta}$ online, as the ill-trained policy is likely to recommend irrelevant items to users. As an alternative solution, the agent can be trained with previously-collected logged data:
\begin{equation}
    \Delta_{\theta}\mathbb{E}_{\tau\sim\beta}\left[\mathcal{R}\left(\tau\right)\right]=
     \mathbb{E}_{\tau\sim\pi_{\theta}}\left[\mathcal{R}\left(\tau\right)\Delta_{\theta}\log\pi_{\theta}\left(\tau\right)\right]
\end{equation}
where $\beta$ denotes the data collection policy (behaviour policy). Obviously, there is a distribution discrepancy between $\beta$ and $\pi_{\theta}$, and it is hard to optimize due to high variance and the difficulty of estimating $\beta$ itself. 

Another successful solution is value-based approaches(e.g., Q-learning~\citep{silver2016mastering}). It utilizes policy evaluation to calculate Q-values $\mathcal{Q}\left(\mathit{s}_{\mathit{t}},\mathit{a}_{\mathit{t}}\right)$ , which is defined as the value of performing a given action $\mathit{a}_{\mathit{t}}$ given the state $\mathit{s}_{\mathit{t}}$. The action is taken by $\mathit{a}_{\mathit{t}}=\argmax\mathcal{Q}(\mathit{s}_{\mathit{t}},\mathit{a})$. The Q-function is trained by minimizing the Bellman Error over Q in a step called policy evaluation:
\begin{equation}
    \mathcal{Q}_{\mathit{i+1}}\leftarrow \mathop\mathit{arg min}_{\substack{\mathcal{Q}}}\mathbb{E}\left[\mathit{r}_{\mathit{t}}+\gamma\mathcal{Q}_{\mathit{i}}(\mathit{s}_{\mathit{t+1}},\mathit{a}_{\mathit{t+1}})-\mathcal{Q}_{\mathit{i}}(\mathit{s}_{\mathit{t}},\mathit{a}_{\mathit{t}})\right]
\end{equation}
where $\mathcal{Q}_{\mathit{i}}$ is the \mathit{i}-th step of policy evaluation. The policy is then trained to maximize the state-action values of performing an action $\mathit{a}_{\mathit{t}}$ given $\mathit{s}_{\mathit{t}}$ in a step called policy improvement:
\begin{equation}
    \pi_{\mathit{i+1}}\leftarrow \mathop\mathit{arg max}_{\substack{\pi}}\mathbb{E}\left[\mathcal{Q}(\mathit{s}_{\mathit{t}},\pi_{\mathit{i}}(\mathit{a}_{\mathit{t}}|\mathit{s}_{\mathit{t}}))\right]
\end{equation}
where $\pi_{\mathit{i}}$ is the \mathit{i}-th step of policy improvement. Similar with the policy gradient-based approaches, we need learn the policy with previously-collected logged data. The policy improvement can now be stated as:
\begin{equation}
    \pi_{\mathit{i+1}}\leftarrow \mathop\mathit{arg max}_{\substack{\pi}}\mathbb{E}_{\mathit{s}_{\mathit{t}}\sim\mathcan{D}}\left[\mathcal{Q}(\mathit{s}_{\mathit{t}},\pi_{\mathit{i}}(\mathit{a}_{\mathit{t}}|\mathit{s}_{\mathit{t}}))\right]
\end{equation}
where \mathcal{D} is the logged data collected by behavior policy $\beta$. In deep reinforcement learning,  the policy and the value functions are parameterized using neural networks and trained using gradient descent.
s
